Valid belief updates for prequentially additive loss functions arising in Semi-Modular Inference

Model-based Bayesian evidence combination leads to models with multiple parameteric modules. In this setting the effects of model misspecification in one of the modules may in some cases be ameliorated by cutting the flow of information from the misspecified module. Semi-Modular Inference (SMI) is a framework allowing partial cuts which modulate but do not completely cut the flow of information between modules. We show that SMI is part of a family of inference procedures which implement partial cuts. It has been shown that additive losses determine an optimal, valid and order-coherent belief update. The losses which arise in Cut models and SMI are not additive. However, like the prequential score function, they have a kind of prequential additivity which we define. We show that prequential additivity is sufficient to determine the optimal valid and order-coherent belief update and that this belief update coincides with the belief update in each of our SMI schemes.

==> notes.tex <==



We then show that our loss functions are additive (in our sense) and coherent using the methods of \cite{carmona20}. It follows that the belief update of \cite{Bissiri2016} applies and so the candidate posterior distributions we consider are valid and coherent.
% The cut model includes Bayesian Multiple Imputation as a special case and so our result taken with that in \cite{carmona20} shows that SMI is a valid belief update.

We discuss belief updates, coherence and additivity in the context of the
two-module model in Fig~\ref{fig:toy_multimodular_model}. This is really just a substantial running example which includes the single module model as a special case. Different dependence structures and further modules may be added.

% Let a prior $\pi_0(\varphi, \theta)$ and a loss function $l(\varphi, \theta;Y,Z,\pi_0)$ be given. The loss function relates the data and parameters. For example, for the model in Fig.~\ref{fig:toy_multimodular_model}, we will see that the loss function which yields the Bayes posterior \eqref{eq:bayespost} is just the negative log-likelihood,
% \begin{equation} \label{eq:bayes_loss}
%   \l^{(b)}( \varphi,\theta ; Y, Z) = - \log p(Z \mid \varphi) -\log p(Y \mid \varphi,\theta).
% \end{equation}
% The loss yielding the Cut model posterior in \eqref{eq:cutpost} will prove to be
% \begin{equation} \label{eq:cut_loss}
%   \l^{(c)}( \varphi,\theta ; Y, Z , \pi_0) = \l^{(b)}( \varphi,\theta ; Y, Z ) + \log p(Y \mid \varphi).
% \end{equation}
% Notice that the loss function for the cut model depends on the prior $\pi(\theta|\varphi)$ through the term $ \log p(Y \mid \varphi)$. There is no prior dependence in the Bayes loss.

% We now define belief updates. These are rules which convert losses, which may be deterministic, into probability distributions expressing a state of knowledge.
% \begin{definition} \label{def:bubasicdef} (Belief Update)
%   A belief update $\psi$ determines an updated probability distribution for the parameters given the data.
%   For the model in Fig.~\ref{fig:toy_multimodular_model}, the update has the form
%   \begin{equation*}
%     \p(\varphi, \theta \mid Y,Z) = \psi\{ l(\varphi, \theta;Y,Z, \pi_0), \pi_0 \}.
%   \end{equation*}
% \end{definition}
% When we specify a probability distribution from a loss, via a belief update, we write it as if it were a conditional probability density. We use $p()$ (for densities over data) and $\pi()$ (for densities over parameters) when it may be understood as a conditional probability. However, many belief updates, such as that for the cut-posterior, do not yield probability distributions which can expanded using conditional probability. We write $\p()$ for probability distributions of this kind.

For any given loss there is a natural \emph{associated belief update} which will prove to be important.
\begin{definition} (associated belief update and loss)
  Let a loss $l(\varphi, \theta;Y,Z, \pi_0)$ be given.
  We refer to
  \begin{equation}\label{eq:beliefupdate}
    \psi\{ l(\varphi, \theta;Y,Z, \pi_0), \pi_0 \}\propto \exp(-l(\varphi, \theta;Y,Z,\pi_0)) \pi_0(\varphi, \theta).
  \end{equation}
  as the candidate belief update \emph{associated with} $l$.
\end{definition}
Association works both ways. A candidate posterior such as the cut posterior determines an associated loss.

We now define additive losses in the setting where the data are independent and identically distributed (iid) given the parameters.
\begin{definition}\label{def:additivity} (Additivity)
  Let $Y=(Y^{(1)},Y^{(2)})$ and $Z=(Z^{(1)},Z^{(2)})$ be arbitrary partitions of each iid data set $Y=(Y_1,...,Y_n)$ and $Z=(Z_1,...,Z_m)$ into two blocks, which may be empty.
  If the loss does not depend on the prior then it is additive if
  \[
    l( \varphi,\theta ; Y, Z ) = l( \varphi,\theta ;Y^{(1)}, Z^{(1)} )+l( \varphi,\theta ; Y^{(2)}, Z^{(2)} )
  \]
  holds for every $n,m>0$ and every partition of the data.
\end{definition}
The Bayes loss $\l^{(b)}$ is additive for iid data. However the cut loss $\l^{(c)}$ is not additive in this sense, due to the term $\log p(Y \mid \varphi)$ - the integral of a product is not equal to the product of integrals. We now define a weaker additivity which does hold for cut models.
\begin{definition}\label{def:preqadd} (Prequential Additivity)
  Let $Y=(Y^{(1)},Y^{(2)})$ and $Z=(Z^{(1)},Z^{(2)})$ be a partition of iid data defined as in Definition~\ref{def:additivity}, let a loss $l( \varphi,\theta ; Y, Z ,\pi_0)$ and a belief update $\psi\{ l(\varphi, \theta;Y,Z,\pi_0),\pi_0\}$ be given and let
  \[
    \pi_1(\varphi, \theta|Y^{(1)},Z^{(1)})=\psi\{ l(\varphi, \theta;Y^{(1)},Z^{(1)},\pi_0),\pi_0\}.
  \]
  The loss $l$ is prequentially additive with respect to the belief update $\psi$ if
  \[
    l( \varphi,\theta ; Y, Z ,\pi_0) = l( \varphi,\theta ;Y^{(1)}, Z^{(1)},\pi_0)+l( \varphi,\theta ; Y^{(2)}, Z^{(2)},  \pi_1), \pi_0)
  \]
  for every partition of iid data taken in any order.
\end{definition}
The point here is that we must update the ``prior'' appearing in the definition of the loss as we accumulate data. The prior for the loss on the second data set is the posterior from the first. The order in which we take the data must not effect the total loss so for example we may take the same partition but swap the labels identifying $Y^{(1)},Z^{(1)}$ and $Y^{(2)},Z^{(2)}$. 

#################################
Proof: We begin with $(\psi,l)=(\psi^{(k)},\l^{(k)})$.
We want to check (d)=(d1)+(d2) in the following diagram.
%TODO - this isnt exactly what the proposition says!

\begin{tikzcd}
  \pi(\varphi,\tilde\theta,\theta) \ar[rr,"(d)", bend left=10] \ar[r,"(d1)", swap] & \p^{(k)}_{\delta}(\varphi,\tilde\theta,\theta \mid Y^{(1)},Z^{(1)}) \ar[r,"(d2)", swap] & \p^{(k)}_{\delta}(\varphi,\tilde\theta,\theta \mid Y,Z)
\end{tikzcd}

The update is
\begin{align*}
  \p_{(d1)}(\varphi,\tilde\theta,\theta) & =\p^{(k)}_{\delta}(\varphi,\tilde\theta,\theta \mid Y^{(1)},Z^{(1)})                                                                                                                                                                                           \\
                                         & \propto p(Z^{(1)} \mid \varphi) p_\delta( Y^{(1)} \mid \varphi, \tilde \theta ) \; p( Y^{(1)} \mid \varphi,  \theta ) \frac{ \pi(\varphi) }{ \int  p( Y^{(1)} \mid \varphi,  \theta ) \; \pi(\varphi, \theta ) \;  d\theta} \pi(\varphi, \tilde\theta, \theta)
\end{align*}
Now we add the data $(Y^{(2)},Z^{(2)})$ but use $\p_{(d1)}(\varphi,\tilde\theta,\theta)$ as the prior.
\begin{align}
  \p_{(d1)+(d2)}(\varphi,\tilde\theta,\theta)
   & \propto  p(Z^{(2)} \mid \varphi)p_\delta( Y^{(2)} \mid \varphi, \tilde \theta ) \; p( Y^{(2)} \mid \varphi,  \theta ) \frac{ \p_{(d1)}(\varphi) }{ \int  p( Y^{(2)} \mid \varphi,  \theta ) \; \p_{(d1)}(\varphi, \theta ) \;  d\theta} \p_{(d1)}(\varphi, \tilde\theta, \theta) \nonumber   \\
   & \propto p(Z^{(2)} \mid \varphi)p_\delta( Y^{(2)} \mid \varphi, \tilde \theta ) \; p( Y^{(2)} \mid \varphi,  \theta ) \frac{ \p_{(d1)}(\varphi) }{ \int  p( Y^{(2)} \mid \varphi,  \theta ) \; \p_{(d1)}(\varphi, \theta ) \;  d\theta}  \nonumber                                            \\
   & \quad \times \quad p(Z^{(1)} \mid \varphi) p_\delta( Y^{(1)} \mid \varphi, \tilde \theta ) \; p( Y^{(1)} \mid \varphi,  \theta ) \frac{ \pi(\varphi) }{ \int  p( Y^{(1)} \mid \varphi,  \theta ) \; \pi(\varphi, \theta ) \;  d\theta} \pi(\varphi, \tilde\theta, \theta) \label{eq:efourks} \\
   & \propto p(Z \mid \varphi) p_\delta(Y \mid \varphi, \tilde\theta ) p(Y  \mid \varphi, \theta )  \pi(\varphi,\tilde\theta,\theta) \nonumber                                                                                                                                                    \\
   & \quad\times\quad \frac{ \p_{(d1)}(\varphi) }{ \int  p( Y^{(2)} \mid \varphi,  \theta ) \; \p_{(d1)}(\varphi, \theta ) \;  d\theta} \frac{ 1 }{ \int  p( Y^{(1)} \mid \varphi,  \theta ) \; \pi(\varphi, \theta ) \;  d\theta } \label{eq:ethreeks}                                           \\
   & \propto p(Z \mid \varphi) p_\delta(Y \mid \varphi, \tilde\theta ) p(Y \mid \varphi, \theta ) \; \frac{1}{ \int  p( Y^{(1)} \mid \varphi,  \theta ) \; \pi(\varphi,\theta) d\theta } \pi(\varphi, \tilde\theta, \theta)\label{eq:etwoks}                                                      \\
   & \propto \p^{(k)}_{\delta}(\varphi,\tilde\theta,\theta \mid Y,Z).\nonumber
\end{align}
We used
\[
  p_\delta(Y \mid \varphi, \tilde\theta )=p_\delta(Y^{(1)} \mid \varphi, \tilde\theta )p_\delta(Y^{(2)} \mid \varphi, \tilde\theta )
\]
to get from \eqref{eq:efourks} to \eqref{eq:ethreeks}. This follows from Eqn.~{\ref{eq:ks-smooth-lkd-prod}} above.
To get from \eqref{eq:ethreeks} to \eqref{eq:etwoks}, we used the following identity
\begin{align*}
  \frac{ \p_{(d1)}(\varphi) }{ \int  p( Y^{(2)} \mid \varphi,  \theta ) \; \p_{(d1)}(\varphi, \theta ) \;  d\theta} & = \frac{ \int \int \p_{(d1)}(\varphi, \tilde\theta, \theta) d\theta d\tilde\theta }{ \int \int p( Y^{(2)} \mid \varphi,  \theta ) \; \p_{(d1)}(\varphi, \tilde\theta, \theta ) \;  d\theta d\tilde\theta}                                                                                                                                                                                                                                                                                                   \\
                                                                                                                    & \propto \frac{ \int \int p_\delta( Y^{(1)} \mid \varphi, \tilde \theta ) \; p( Y^{(1)} \mid \varphi,  \theta ) \frac{1}{ p(Y^{(1)} \mid \varphi)_{\theta} } \pi(\varphi, \tilde\theta, \theta) d\theta d\tilde\theta }{ \int \int p( Y^{(2)} \mid \varphi,  \theta ) \; p_\delta( Y^{(1)} \mid \varphi, \tilde \theta ) \; p( Y^{(1)} \mid \varphi,  \theta ) \frac{1}{ p(Y^{(1)} \mid \varphi)_{\theta} } \pi(\varphi, \tilde\theta, \theta) \;  d\theta d\tilde\theta}                                    \\
                                                                                                                    & = \frac{ \frac{1}{\pi(\varphi)} \left( \int p_\delta( Y^{(1)} \mid \varphi, \tilde \theta ) \pi(\varphi,\tilde\theta) d\tilde\theta \right) \left(\int  p( Y^{(1)} \mid \varphi,  \theta ) \pi(\varphi,\theta) d\theta \right) }{ \frac{1}{\pi(\varphi)} \left( \int  p_\delta( Y^{(1)} \mid \varphi, \tilde \theta ) \pi(\varphi,\tilde\theta) \;  d\tilde\theta \right) \left(  \int p( Y^{(1)} \mid \varphi,  \theta ) p( Y^{(2)} \mid \varphi,  \theta ) \; \pi(\varphi, \theta ) \;  d\theta \right) } \\
                                                                                                                    & =\frac{ p(Y^{(1)} \mid \varphi)_{\theta} }{ p(Y \mid \varphi)_{\theta} }.
\end{align*}
Here we assumed that $\theta$ and $\tilde\theta$ are conditionally independent given $\varphi$ in the prior, so $ \pi(\varphi, \tilde\theta, \theta) = p( \varphi, \theta ) \; p( \varphi, \tilde\theta ) \frac{1}{\pi(\varphi)} $.

We next verify the result for the update with $(\psi,l)=(\psi^{(t)},\l^{(t)})$. In this setting we want to check the $(e)=(e1)+(e2)$ update in the following diagram.

\begin{tikzcd}
  \pi(\varphi,\tilde\theta,\theta) \ar[rr,"(e)", bend left=10] \ar[r,"(e1)", swap] & \p^{(t)}_\gamma(\varphi,\theta \mid Y^{(1)},Z^{(1)}) \ar[r,"(e2)", swap] & \p^{(t)}_\gamma(\varphi,\theta \mid Y,Z)
\end{tikzcd}
Starting from \eqref{eq:gamma_smi_post_tmp},
%WORK INP PROGRESS BELOW!!
\begin{align}
  \p_{(e1)}(\varphi,\theta \mid Y^{(1)},Z^{(1)}) & \propto  p(Z^{(1)}|\varphi)p(Y^{(1)} \mid \varphi,\theta ) \; \frac{1}{p(Y^{(1)} \mid \varphi)_\theta^{1-\gamma} } \pi(\varphi,\theta) \nonumber                                                                                                                            \\
                                                 & \propto p(Z^{(1)}|\varphi)p(Y^{(1)} \mid \varphi,\theta ) \; \frac{\pi(\varphi)^{1-\gamma}}{ \left[\int p(Y^{(1)}|\varphi,\theta)\pi(\varphi, \theta)d\theta\right]^{1-\gamma}} \pi(\varphi,\theta) \nonumber                                                               \\
  \p_{(e1)+(e2)}(\varphi,\theta,\mid Y^{(1)},Z^{(1)},(Y^{(2)},Z^{(2)}))
                                                 & \propto  p(Z^{(2)}|\varphi)p(Y^{(2)} \mid \varphi,\theta ) \; \frac{\p_{(e1)}(\varphi)^{1-\gamma}}{ \left[\int p(Y^{(2)}|\varphi,\theta')\p_{(e1)}(\theta',\varphi)d\theta'\right]^{1-\gamma}} \p_{(e1)}(\varphi, \theta) \nonumber                                         \\
                                                 & \propto  p(Z|\varphi)p(Y \mid \varphi, \theta ) \pi(\varphi,\theta)\cdot\nonumber                                                                                                                                                                                           \\
                                                 & \cdot\frac{ [\p_{(e1)}(\varphi) \pi(\varphi)]^{1-\gamma}}{ \left[\int  p( Y^{(2)} \mid \varphi,  \theta' ) \; \p_{(e1)}(\varphi, \theta' ) \;  d\theta' \int  p( Y^{(1)} \mid \varphi,  \theta ) \; \pi(\varphi, \theta ) \;  d\theta\right]^{1-\gamma}}  \label{eq:ethree} \\
                                                 & \propto \pi(\varphi,\theta|Y,Z)\frac{\pi(\varphi)^{1-\gamma}}{\left[\int  p( Y \mid \varphi,  \theta ) \; \pi(\varphi, \theta ) \;  d\theta \right]^{1-\gamma}}\label{eq:etwo}                                                                                              \\
                                                 & \propto \p^{(t)}_{\gamma}(\varphi,\theta|Y,Z).\nonumber
\end{align}
In the step from \eqref{eq:ethree} to \eqref{eq:etwo}, we used the following identity
\begin{align*}
  \frac{ \p_{(e1)}(\varphi) }{ \int  p( Y^{(2)} \mid \varphi,  \theta' ) \; \p_{(e1)}(\varphi, \theta' ) \;  d\theta'  }
   & = \frac{ \int p(Z^{(1)}|\varphi)p(Y^{(1)} \mid \varphi,\theta ) \; \frac{\pi(\varphi)^{1-\gamma}}{ \left[\int p(Y^{(1)}|\varphi,\theta)\pi(\varphi, \theta)d\theta\right]^{1-\gamma}} \pi(\varphi,\theta)d\theta }{ \int p( Y^{(2)} \mid \varphi,  \theta' ) \; p(Z^{(1)}|\varphi)p(Y^{(1)} \mid \varphi,\theta' ) \; \frac{\pi(\varphi)^{1-\gamma}}{ \left[\int p(Y^{(1)}|\varphi,\theta)\pi(\varphi, \theta)d\theta\right]^{1-\gamma}} \pi(\varphi,\theta')d\theta'} \\
   & =\frac{ \int  p( Y^{(1)} \mid \varphi,  \theta ) \; \pi(\varphi, \theta ) \;  d\theta }{ \int  p( Y \mid \varphi,  \theta' ) \; \pi(\varphi, \theta' ) \;  d\theta' }
\end{align*}

[EOP]

% \subsection{Additivity of the loss}

% Our definition of order coherence in \eqref{eq:order-coherent} differs from that given in \cite{Bissiri2016}.
% We have \eqref{eq:order-coherent} whilst they have
% \begin{equation}\label{eq:order-coherent-BHW}
%   \psi\{ l(\varphi,\theta;Y^{(2)},Z^{(2)}) , \pi_1 \} \} = \psi\{ l(\varphi,\theta;Y^{(1)},Z^{(1)})+l(\varphi,\theta;Y^{(2)},Z^{(2)}), \pi_0 \},
% \end{equation}
% where $\pi_0=\pi(\varphi,\theta)$ is the ``original" prior, and $\pi_1$ is
% \[
% \pi_1=\psi\{ l(\varphi,\theta;Y^{(1)},Z^{(1)}) , \pi_0\},
% \]
% the ``updated" prior after the arrival of the data $Y^{(1)},Z^{(1)}$.

% There are two points of difference. First we emphasise the point made in \eqref{eq:cut_loss_prior_dep} that the prior $\pi_0$ and the updated prior $\pi_1$ may appear in the loss, so we have $l(\varphi,\theta;Y^{(1)},Z^{(1)},\pi_0)$ and $l(\varphi,\theta;Y^{(2)},Z^{(2)},\pi_1)$ etc.
% Wherever a prior appears in the second stage it must be equal to the posterior for the first stage. Operationally this is what we must do as we ``apply the same rule" at each stage.

% The second point which is the subject of this section is that
%  the right hand side of \eqref{eq:order-coherent} we write the loss for the full data set $l(\varphi,\theta;Y,Z,\pi_0)$
% where \cite{Bissiri2016} write $l(\varphi,\theta;Y^{(1)},Z^{(1)})+l(\varphi,\theta;Y^{(2)},Z^{(2)})$. These are equal if the loss is additive.
% Writing $l(\varphi,\theta;Y^{(1)},Z^{(1)})+l(\varphi,\theta;Y^{(2)},Z^{(2)})$ does not seem to be necessary or even desirable. The Cut-model loss is not additive but is nevertheless order-coherent in the sense of \eqref{eq:order-coherent}, as \cite{carmona20} have shown. Furthermore we must operationally have the loss on the full data on the right, as this is the posterior for the full data and what we actually compute when we apply the update rule.
% There is a question over whether the order-coherence we have shown in Sec~\ref{sec:oc}

% so we cannot immediately claim the belief update in \eqref{eq:beliefupdate} is the unique valid and coherent update.
% We will have
% \begin{equation}
%     l(\varphi,\theta;Y,Z)=l(\varphi,\theta;Y^{(2)},Z^{(2)})
%         + l(\varphi,\theta;Y^{(2)},Z^{(2)})
% \end{equation}

% Also, on




% valid (in the sense of \cite{Bissiri2016}) and give
